Global Transport Couplings for Classifier-Free Guided Flows

Optimal-transport couplings have been shown to reduce training variance in unconditional flow models, but their role in conditional generation remains unclear. A natural approach constructs separate couplings for each condition, but this is impractical for large or continuous conditioning spaces found in modern image foundation models. We introduce Global Transport (GT), a global class-agnostic optimal-transport coupling, computed without class labels. GT can associate different conditions with different regions of the source noise, and consequently worsens performance without guidance. However, when combined with classifier-free guidance (CFG), GT consistently improves generation across domains, model scales, and sampling budgets. This reversal suggests that couplings for conditional flows should be evaluated both empirically and theoretically under the guided flow used at inference, rather than on unguided generation. We evaluate GT over both discrete class and continuous text conditioned image generation across model scales, and investigate how coupling choice alters guided trajectories. These results identify coupling design in the guided flow setting as a simple training time axis to improve performance without modifying existing architectures, samplers, or guidance mechanisms.

==> b2_case_study.tex <==
% =========================================================
% B/2 PANEL
% =========================================================
\begin{minipage}[t]{0.39\textwidth}
\vspace{0pt}
\centering
\small
\setlength{\tabcolsep}{3pt}

% ---------------------------------------------------------
% TOP PANEL
% ---------------------------------------------------------
\resizebox{\linewidth}{!}{%
\begin{tabular}{@{}lccc@{}}
\toprule
Coupling $\downarrow$ / Steps $\rightarrow$
& 16 & 32 & 64 \\
\midrule
Independent
& 5.88 & 5.32 & 5.22 \\
Global Transport
& \textbf{5.15} & \textbf{4.35} & \textbf{4.14} \\
Class-conditional OT
& 5.79 & 5.20 & 5.08 \\
\bottomrule
\end{tabular}%
}

\vspace{1.0em}

% ---------------------------------------------------------
% BOTTOM PANEL
% ---------------------------------------------------------
\resizebox{\linewidth}{!}{%
\begin{tabular}{@{}lccc@{}}
\toprule
Coupling $\downarrow$ / Steps $\rightarrow$
& 1 & 2 & 4 \\
\midrule
Independent
& 5.82 & 5.19 & 5.19 \\
Global Transport
& \textbf{5.66} & \textbf{4.17} & \textbf{4.14} \\
Global Transport (finetune)
& 5.88 & 4.21 & 4.18 \\
\bottomrule
\end{tabular}%
}

\end{minipage}

==> cfg_ablation.tex <==
\begin{table*}[h]
\label{tab:cfg_sweep_ablation}
\centering
\caption{FID as a function of guidance scale $w$ for SiT-XL/2 with 64 Euler steps.}
\label{tab:guidance-scale}
\begin{tabular}{l *{7}{c}}
\toprule
Coupling $\downarrow$ \;/\; $w \rightarrow$
& 1.0 & 1.5 & 2.0 & 2.5 & 3.0 & 3.5 & 4.0 \\
\midrule
Independent
& 12.58 & 2.78 & 6.10 & 10.41 & 13.76 & 16.14 & 17.87 \\
\quad + Guidance interval $[0, 0.7]$
& 12.58 & 3.96 & 2.16 & 2.63 & 3.73 & 4.93 & 6.04 \\
% \quad + CFG-Zero$\star$
% & -- & -- & -- & -- & -- & -- & -- \\
% \quad + Autoguidance
% & -- & -- & -- & -- & -- & -- & -- \\
\midrule
Global Transport
& 16.11 & 2.63 & 3.87 & 7.47 & 10.70 & 13.16 & 15.09 \\
\quad + Guidance interval $[0, 0.7]$
& 16.11 & 5.89 & 2.61 & 2.01 & 2.40 & 3.12 & 3.91 \\
% \quad + CFG-Zero$\star$
% & -- & -- & -- & -- & -- & -- & -- \\
% \quad + Autoguidance
% & -- & -- & -- & -- & -- & -- & -- \\
\bottomrule
\end{tabular}%
\end{table*}


==> cfg_sweep.tex <==
% \begin{table*}[h]
% \caption{\small \textbf{Left:} FID\,$\downarrow$ on ImageNet-256 for independent, class-conditional OT and \gt couplings across SiT scales (B/2, L/2, XL/2: 130M, 459M, 675M parameters), sampling steps and guidance scales $w$. \textbf{Right:} FID\,$\downarrow$ vs.\ $w$ for SiT-XL/2 (64 Euler steps) under the full guidance interval (Full) and a tuned interval $[0,0.7]$ (GI).}
% \label{tab:sit_ablations}\label{tab:cfg_sweep_ablation}
% \centering
% \scriptsize
% \setlength{\tabcolsep}{2.5pt}
% \begin{minipage}[c]{0.71\textwidth}
% \centering
% \begin{tabular}{ll *{9}{c}}
% \toprule
%  & & \multicolumn{3}{c}{16 steps} & \multicolumn{3}{c}{32 steps} & \multicolumn{3}{c}{64 steps} \\
% \cmidrule(lr){3-5}\cmidrule(lr){6-8}\cmidrule(lr){9-11}
% Model & Coupling & $w{=}1.0$ & 2.0 & 4.0 & 1.0 & 2.0 & 4.0 & 1.0 & 2.0 & 4.0 \\
% \midrule
% \multirow{3}{*}{SiT-B/2}
%  & Independent     & 33.29 & 5.88 & 15.37 & 28.33 & 5.32 & 15.78 & 26.58 & 5.22 & 15.84 \\
%  & Class-cond.\ OT & 33.18 & 5.79 & 15.15 & 28.43 & 5.20 & 15.59 & 26.72 & 5.08 & 15.59 \\
%  & SD-OT & 56.98 & 12.21 & 5.57 & 53.30 & 11.31 & 5.44 & 52.01 & 11.04 & 5.41 \\ 
%  & SD-OT (model space) & 48.89 & 9.01 & 5.61 & 44.98 & 8.06 &  15.59 & 26.72 & 5.08 & 15.59 \\
%  & \gt             & 38.08 & \textbf{5.15} & 13.24 & 33.27 & \textbf{4.35} & 13.49 & 31.43 & \textbf{4.14} & 13.54 \\
% \midrule
% \multirow{3}{*}{SiT-L/2}
%  & Independent     & 19.53 & 5.50 & 17.56 & 15.30 & 5.74 & 17.86 & 13.85 & 5.85 & 17.89 \\
%  & Class-cond.\ OT & 19.61 & 5.47 & 17.28 & 15.47 & 5.68 & 17.71 & 13.96 & 5.81 & 17.79 \\
%  & \gt             & 23.77 & \textbf{3.94} & 14.76 & 19.35 & \textbf{3.84} & 15.17 & 17.72 & \textbf{3.88} & 15.17 \\
% \midrule
% \multirow{2}{*}{SiT-XL/2}
%  & Independent     & 18.57 & 5.55 & 17.53 & 14.26 & 5.89 & 17.80 & 12.58 & 6.10 & 17.87 \\
%  & \gt             & 22.44 & \textbf{3.87} & 14.66 & 17.82 & \textbf{3.82} & 15.03 & 16.11 & \textbf{3.87} & 15.09 \\
% \bottomrule
% \end{tabular}
% \end{minipage}\hfill
% \begin{minipage}[c]{0.27\textwidth}
% \centering
% \renewcommand{\arraystretch}{1.12}
% \begin{tabular}{c cc cc}
% \toprule
%  & \multicolumn{2}{c}{Independent} & \multicolumn{2}{c}{\gt} \\
% \cmidrule(lr){2-3}\cmidrule(lr){4-5}
% $w$ & Full & GI & Full & GI \\
% \midrule
% 1.0 & \textbf{12.58} & \textbf{12.58} & 16.11 & 16.11 \\
% 1.5 &  2.78 &  3.96 & \textbf{2.63} &  5.89 \\
% 2.0 &  6.10 & \textbf{2.16} &  3.87 &  2.61 \\
% 2.5 & 10.41 &  2.63 &  7.47 & \textbf{2.01} \\
% 3.0 & 13.76 &  3.73 & 10.70 & \textbf{2.40} \\
% 3.5 & 16.14 &  4.93 & 13.16 & \textbf{3.12} \\
% 4.0 & 17.87 &  6.04 & 15.09 & \textbf{3.91} \\
% \bottomrule
% \end{tabular}
% \end{minipage}
% \end{table*}
% \begin{figure}[h]
%     \centering
%     \includegraphics[width=\linewidth]{figs/imagenet/cfg_sweep_sit_ot_vs_ind_xl_2_256_seed5_paper_2rows_w1-6.png}
%     \caption{Caption}
%     \label{fig:placeholder}
% \end{figure}

\newcommand{\wsel}[1]{\,{\tiny($#1$)}}

% \begin{table*}[h]
% \caption{\small FID\,$\downarrow$ and FD\textsubscript{DINOv2}\,$\downarrow$ on ImageNet-256 for independent, class-conditional OT and \gt couplings across SiT scales (B/2, L/2, XL/2: 130M, 459M, 675M parameters) and sampling steps, under the full guidance interval. Each entry reports the best value over the guidance scales $w$ evaluated (Tables~2, 6 and 7), selected separately for each metric; the selected $w$ is given in parentheses.}
% \label{tab:sit_best_w}
% \centering
% \scriptsize
% \setlength{\tabcolsep}{4pt}
% \begin{tabular}{ll ccc ccc}
% \toprule
%  & & \multicolumn{3}{c}{FID\,$\downarrow$} & \multicolumn{3}{c}{FD\textsubscript{DINOv2}\,$\downarrow$} \\
% \cmidrule(lr){3-5}\cmidrule(lr){6-8}
% Model & Coupling & 16 steps & 32 steps & 64 steps & 16 steps & 32 steps & 64 steps \\
% \midrule
% \multirow{5}{*}{SiT-B/2}
%  & Independent              & 5.88\wsel{2.0} & 5.32\wsel{2.0} & 5.22\wsel{2.0} & 137.3\wsel{4.0} & 132.9\wsel{4.0} & 131.9\wsel{4.0} \\
%  & Class-cond.\ OT          & 5.79\wsel{2.0} & 5.20\wsel{2.0} & 5.08\wsel{2.0} & 136.4\wsel{4.0} & 132.2\wsel{4.0} & 131.4\wsel{4.0} \\
%  & \gt-SD-OT                & 5.57\wsel{4.0} & 5.44\wsel{4.0} & 5.41\wsel{4.0} & -- & -- & -- \\
%  & \gt-SD-OT (model space)  & 5.61\wsel{4.0} & 5.52\wsel{4.0} & 5.49\wsel{4.0} & -- & -- & -- \\
%  & \gt                      & \textbf{5.15}\wsel{2.0} & \textbf{4.35}\wsel{2.0} & \textbf{4.14}\wsel{2.0} & \textbf{123.6}\wsel{4.0} & \textbf{118.0}\wsel{4.0} & \textbf{116.8}\wsel{4.0} \\
% \midrule
% \multirow{3}{*}{SiT-L/2}
%  & Independent              & 5.50\wsel{2.0} & 5.74\wsel{2.0} & \textbf{2.95}\wsel{1.5} & 91.1\wsel{2.5} & 84.6\wsel{2.5} & 83.3\wsel{2.5} \\
%  & Class-cond.\ OT          & 5.47\wsel{2.0} & 5.68\wsel{2.0} & 5.81\wsel{2.0} & 102.0\wsel{4.0} & 99.2\wsel{2.0} & 95.0\wsel{2.0} \\
%  & \gt                      & \textbf{3.94}\wsel{2.0} & \textbf{3.84}\wsel{2.0} & 2.96\wsel{1.5} & \textbf{83.5}\wsel{4.0} & \textbf{78.7}\wsel{2.5} & \textbf{73.5}\wsel{3.0} \\
% \midrule
% \multirow{2}{*}{SiT-XL/2}
%  & Independent              & 3.95\wsel{1.5} & 3.00\wsel{1.5} & 2.78\wsel{1.5} & 84.2\wsel{2.5} & 78.7\wsel{2.5} & 77.8\wsel{2.5} \\
%  & \gt                      & \textbf{3.22}\wsel{1.75} & \textbf{2.69}\wsel{1.75} & \textbf{2.59}\wsel{1.75} & \textbf{72.7}\wsel{3.0} & \textbf{69.1}\wsel{3.0} & \textbf{68.4}\wsel{3.0} \\
% \bottomrule
% \end{tabular}
% \end{table*}

% \begin{table*}[h]
% \caption{\small FID and FD\textsubscript{DINOv2} on ImageNet-256 across SiT scales, couplings, and sampling steps.}
% \label{tab:sit_best_w}
% \centering
% \scriptsize
% \setlength{\tabcolsep}{4pt}
% \begin{tabular}{ll ccc ccc}
% \toprule
% \multirow{2}{*}{Model} & \multirow{2}{*}{Coupling}
% & \multicolumn{3}{c}{FID\,$\downarrow$}
% & \multicolumn{3}{c}{FD\textsubscript{DINOv2}\,$\downarrow$} \\
% \cmidrule(lr){3-5}\cmidrule(lr){6-8}
% & & 16 & 32 & 64 & 16 & 32 & 64 \\
% \midrule
% \multirow{4}{*}{\shortstack[l]{SiT-B/2\\(130M)}}
% & Independent             & 5.88 & 5.32 & 5.22 & 137.3 & 132.9 & 131.9 \\
% & Class-cond.\ OT         & 5.79 & 5.20 & 5.08 & 136.4 & 132.2 & 131.4 \\
% & \gt + SD-OT               & 5.57 & 5.44 & 5.41 & -- & -- & -- \\
% %& \gt + SD-OT (model space) & 5.61 & 5.52 & 5.49 & -- & -- & -- \\
% & \gt                     & \textbf{5.15} & \textbf{4.35} & \textbf{4.14}
%                           & \textbf{123.6} & \textbf{118.0} & \textbf{116.8} \\
% \midrule
% \multirow{3}{*}{\shortstack[l]{SiT-L/2\\(459M)}}
% & Independent             & 5.50 & 5.74 & 2.95 & 91.1 & 84.6 & 83.3 \\
% & Class-cond.\ OT         & 5.47 & 5.68 & 5.81 & 102.0 & 99.2 & 95.0 \\
% & \gt                     & \textbf{3.94} & \textbf{3.84} & \textbf{2.69}
%                           & \textbf{83.5} & \textbf{78.7} & \textbf{73.5} \\
% \midrule
% \multirow{2}{*}{\shortstack[l]{SiT-XL/2\\(675M)}}
% & Independent             & 3.95 & 3.00 & 2.78 & 84.2 & 78.7 & 77.8 \\
% & \gt                     & \textbf{3.22} & \textbf{2.69} & \textbf{2.59}
%                           & \textbf{72.7} & \textbf{69.1} & \textbf{68.4} \\
% \bottomrule
% \end{tabular}
% \end{table*}

\begin{table*}[h]
\caption{\small FID and FD\textsubscript{DINOv2} on ImageNet-256 across SiT scales, couplings, and sampling steps.}
\label{tab:sit_best_w}
\centering
\scriptsize
\setlength{\tabcolsep}{3pt}
\resizebox{\textwidth}{!}{%
\begin{tabular}{ll cccc cccc cccc cccc}
\toprule
\multirow{2}{*}{Model} & \multirow{2}{*}{Coupling}
& \multicolumn{4}{c}{Euler-16}
& \multicolumn{4}{c}{Euler-32}
& \multicolumn{4}{c}{Euler-64}
& \multicolumn{4}{c}{Dopri5} \\
\cmidrule(lr){3-6}\cmidrule(lr){7-10}\cmidrule(lr){11-14}\cmidrule(lr){15-18}
& & CFG & FID\,$\downarrow$ & CFG & FD\textsubscript{DINOv2}\,$\downarrow$
  & CFG & FID\,$\downarrow$ & CFG & FD\textsubscript{DINOv2}\,$\downarrow$
  & CFG & FID\,$\downarrow$ & CFG & FD\textsubscript{DINOv2}\,$\downarrow$
  & CFG & FID\,$\downarrow$ & CFG & FD\textsubscript{DINOv2}\,$\downarrow$ \\
\midrule
\multirow{4}{*}{\shortstack[l]{SiT-B/2\\(130M)}}
& Independent
  & 2.0 & 5.88 & 4.0 & 137.3
  & 2.0 & 5.33 & 4.0 & 132.9
  & 2.0 & 5.16 & 4.0 & 132.3
  & 2.0 & 5.17 & 4.0 & 132.9 \\
& Class-cond.\ OT
  & 2.0 & 5.79 & 4.0 & 136.4
  & 2.0 & 5.20 & 4.0 & 132.2
  & 2.0 & 5.08 & 4.0 & 131.4
  & -- & -- & -- & -- \\
& \gt + SD-OT
  & -- & 5.57 & -- & --
  & -- & 5.44 & -- & --
  & -- & 5.41 & -- & --
  & -- & -- & -- & -- \\
& \gt
  & 2.0 & \textbf{5.15} & 4.0 & \textbf{123.6}
  & 2.0 & \textbf{4.35} & 4.0 & \textbf{118.0}
  & 2.0 & \textbf{4.15} & 4.0 & \textbf{116.4}
  & 2.0 & \textbf{4.06} & 4.0 & \textbf{116.3} \\
%& \gt + SD-OT (model space)
%  & -- & 5.61 & -- & --
%  & -- & 5.52 & -- & --
%  & -- & 5.49 & -- & --
%  & -- & -- & -- & -- \\
\midrule
\multirow{3}{*}{\shortstack[l]{SiT-L/2\\(459M)}}
& Independent
  & 2.0 & 5.50 & 2.5 & 91.1
  & 2.0 & 5.74 & 2.5 & 84.6
  & 1.5 & 2.95 & 2.5 & 83.3
  & 2.0 & 6.01 & 2.0 & 92.9 \\
& Class-cond.\ OT
  & 2.0 & 5.47 & 4.0 & 102.0
  & 2.0 & 5.68 & 2.0 & 99.2
  & 1.5 & 2.98 & 2.0 & 95.0
  & -- & -- & -- & -- \\
& \gt
  & 2.0 & \textbf{3.94} & 4.0 & \textbf{83.5}
  & 2.0 & \textbf{3.84} & 2.5 & \textbf{78.7}
  & 1.75 & \textbf{2.69} & 3.0 & \textbf{73.5}
  & 2.0 & \textbf{3.98} & 4.0 & \textbf{84.4} \\
\midrule
\multirow{2}{*}{\shortstack[l]{SiT-XL/2\\(675M)}}
& Independent
  & 1.5 & 3.95 & 2.5 & 84.2
  & 1.5 & 3.00 & 2.5 & 78.7
  & 1.5 & 2.78 & 2.5 & 77.8
  & -- & -- & -- & -- \\
& \gt
  & 1.75 & \textbf{3.22} & 3.0 & \textbf{72.7}
  & 1.75 & \textbf{2.69} & 3.0 & \textbf{69.1}
  & 1.75 & \textbf{2.59} & 3.0 & \textbf{68.4}
  & -- & -- & -- & -- \\
\bottomrule
\end{tabular}}
\end{table*}


\begin{figure}[h]
    \centering
    \begin{minipage}[b]{0.49\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figs/imagenet/imagenet_fid_cfg_semidiscrete.pdf}\\[2pt]
        {\small (a) Full guidance interval}
    \end{minipage}\hfill
    \begin{minipage}[b]{0.49\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figs/imagenet/imagenet_fid_cfg_semidiscrete_gi.pdf}\\[2pt]
        {\small (b) Tuned guidance interval $[0.1, 0.7]$}
    \end{minipage}
    \caption{FID\,$\downarrow$ vs.\ guidance scale $w$ for SiT-B/2 (64 Euler steps) under (a) the full guidance interval and (b) a tuned guidance interval.}
    \label{fig:fid_cfg}
\end{figure}

% \begin{table*}[h]
% \caption{\small FID\,$\downarrow$ vs.\ guidance scale $w$ for independent and \gt couplings across SiT scales (64 Euler steps), under the full guidance interval (Full) and a tuned interval (GI): $[0.1, 0.7]$ for B/2 and $[0, 0.7]$ for L/2 and XL/2. At $w{=}1.0$ guidance is inactive, so both settings coincide. \textbf{Bold}: better coupling per column within each model. \underline{Underline}: best $w$ per row within Full and within GI.}
% \label{tab:gi_sweep}
% \centering
% \scriptsize
% \setlength{\tabcolsep}{3.5pt}
% \begin{tabular}{ll c ccccc ccccc}
% \toprule
%  & & & \multicolumn{5}{c}{Full} & \multicolumn{5}{c}{GI} \\
% \cmidrule(lr){4-8}\cmidrule(lr){9-13}
% Model & Coupling & $w{=}1.0$ & 1.5 & 2.0 & 2.5 & 3.0 & 4.0 & 1.5 & 2.0 & 2.5 & 3.0 & 4.0 \\
% \midrule
% \multirow{2}{*}{SiT-B/2}
%  & Independent & \textbf{26.44} & \textbf{6.68} & \underline{5.16} & 7.93 & 11.04 & 15.76 & \textbf{12.14} & \textbf{6.12} & \textbf{4.02} & \underline{3.68} & 4.89 \\
%  & \gt         & 31.16 & 8.13 & \underline{\textbf{4.15}} & \textbf{5.88} & \textbf{8.72} & \textbf{13.41} & 15.89 & 8.29 & 4.88 & \underline{\textbf{3.58}} & \textbf{3.59} \\
% \midrule
% \multirow{2}{*}{SiT-L/2}
%  & Independent & \textbf{13.85} & \underline{\textbf{2.95}} & 5.85 & 10.10 & 13.53 & 17.89 & \textbf{4.53} & \underline{\textbf{2.35}} & 2.62 & 3.65 & 6.00 \\
%  & \gt         & 17.72 & \underline{2.96} & \textbf{3.88} & \textbf{7.38} & \textbf{10.66} & \textbf{15.17} & 6.64 & 2.96 & \underline{\textbf{2.17}} & \textbf{2.48} & \textbf{4.02} \\
% \midrule
% \multirow{2}{*}{SiT-XL/2}
%  & Independent & \textbf{12.58} & \underline{2.78} & 6.10 & 10.41 & 13.76 & 17.87 & \textbf{3.96} & \underline{\textbf{2.16}} & 2.63 & 3.73 & 6.04 \\
%  & \gt         & 16.11 & \underline{\textbf{2.63}} & \textbf{3.87} & \textbf{7.47} & \textbf{10.70} & \textbf{15.09} & 5.89 & 2.61 & \underline{\textbf{2.01}} & \textbf{2.40} & \textbf{3.91} \\
% \bottomrule
% \end{tabular}
% \end{table*}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.98\linewidth]{figs/imagenet/imagenet_metrics_nfe_cfg.pdf}
    \caption{Dopri5}
    \label{fig: dopri5}
\end{figure}

==> cfgg_sweep_horse.tex <==
\begin{table*}[h]
\caption{\small \textbf{Top left:} FID\,$\downarrow$ on ImageNet-256 for independent, class-conditional OT and \gt couplings across SiT scales (B/2, L/2, XL/2: 130M, 459M, 675M parameters), sampling steps and guidance scales $w$. \textbf{Top right / bottom right:} FID\,$\downarrow$ vs.\ $w$ for SiT-XL/2 and SiT-L/2 (64 Euler steps) under the full guidance interval (Full) and a tuned interval $[0,0.7]$ (GI). \textbf{Bottom left:} SiT-XL/2 samples for fixed noise and class as $w$ increases, under \gt (top) and the independent coupling (bottom): \gt refines within a mode, the independent coupling jumps to a different one.}
\label{tab:sit_ablations}\label{tab:cfg_sweep_ablation}\label{fig:mode_stability}
\centering
\scriptsize
\setlength{\tabcolsep}{2.5pt}
%% ---------- top row ----------
\begin{minipage}[c]{0.71\textwidth}
\centering
\begin{tabular}{ll *{9}{c}}
\toprule
 & & \multicolumn{3}{c}{16 steps} & \multicolumn{3}{c}{32 steps} & \multicolumn{3}{c}{64 steps} \\
\cmidrule(lr){3-5}\cmidrule(lr){6-8}\cmidrule(lr){9-11}
Model & Coupling & $w{=}1.0$ & 2.0 & 4.0 & 1.0 & 2.0 & 4.0 & 1.0 & 2.0 & 4.0 \\
\midrule
\multirow{3}{*}{SiT-B/2}
 & Independent     & 33.29 & 5.88 & 15.37 & 28.33 & 5.32 & 15.78 & 26.58 & 5.22 & 15.84 \\
 & \gt             & 38.08 & \textbf{5.15} & 13.24 & 33.27 & \textbf{4.35} & 13.49 & 31.43 & \textbf{4.14} & 13.54 \\
 & Class-cond.\ OT & 33.18 & 5.79 & 15.15 & 28.43 & 5.20 & 15.59 & 26.72 & 5.08 & 15.59 \\
\midrule
\multirow{3}{*}{SiT-L/2}
 & Independent     & 19.53 & 5.50 & 17.56 & 15.30 & 5.74 & 17.86 & 13.85 & 5.85 & 17.89 \\
 & \gt             & 23.77 & \textbf{3.94} & 14.76 & 19.35 & \textbf{3.84} & 15.17 & 17.72 & \textbf{3.88} & 15.17 \\
 & Class-cond.\ OT & 19.61 & 5.47 & 17.28 & 15.47 & 5.68 & 17.71 & 13.96 & 5.81 & 17.79 \\
\midrule
\multirow{2}{*}{SiT-XL/2}
 & Independent     & 18.57 & 5.55 & 17.53 & 14.26 & 5.89 & 17.80 & 12.58 & 6.10 & 17.87 \\
 & \gt             & 22.44 & \textbf{3.87} & 14.66 & 17.82 & \textbf{3.82} & 15.03 & 16.11 & \textbf{3.87} & 15.09 \\
\bottomrule
\end{tabular}
\end{minipage}\hfill
\begin{minipage}[c]{0.27\textwidth}
\centering
\renewcommand{\arraystretch}{1.12}
\begin{tabular}{c cc cc}
\toprule
\multicolumn{5}{c}{SiT-XL/2} \\
\midrule
 & \multicolumn{2}{c}{Independent} & \multicolumn{2}{c}{\gt} \\
\cmidrule(lr){2-3}\cmidrule(lr){4-5}
$w$ & Full & GI & Full & GI \\
\midrule
1.0 & \textbf{12.58} & \textbf{12.58} & 16.11 & 16.11 \\
1.5 &  2.78 &  3.96 & \textbf{2.63} &  5.89 \\
2.0 &  6.10 & \textbf{2.16} &  3.87 &  2.61 \\
2.5 & 10.41 &  2.63 &  7.47 & \textbf{2.01} \\
3.0 & 13.76 &  3.73 & 10.70 & \textbf{2.40} \\
3.5 & 16.14 &  4.93 & 13.16 & \textbf{3.12} \\
4.0 & 17.87 &  6.04 & 15.09 & \textbf{3.91} \\
\bottomrule
\end{tabular}
\end{minipage}

\vspace{6pt}

%% ---------- bottom row ----------
\sbox{\tablebox}{%
\renewcommand{\arraystretch}{1.12}%
\begin{tabular}{c cc cc}
\toprule
\multicolumn{5}{c}{SiT-L/2} \\
\midrule
 & \multicolumn{2}{c}{Independent} & \multicolumn{2}{c}{\gt} \\
\cmidrule(lr){2-3}\cmidrule(lr){4-5}
$w$ & Full & GI & Full & GI \\
\midrule
1.0 & \textbf{13.85} & \textbf{13.85} & 17.72 & 17.72 \\
1.5 & \textbf{2.95} &  4.53 &  2.96 &  6.64 \\
2.0 &  5.85 & \textbf{2.35} &  3.88 &  2.96 \\
2.5 & 10.10 &  2.62 &  7.38 & \textbf{2.17} \\
3.0 & 13.53 &  3.65 & 10.66 & \textbf{2.48} \\
3.5 & 16.03 &  4.84 & 13.25 & \textbf{3.20} \\
4.0 & 17.89 &  6.00 & 15.17 & \textbf{4.02} \\
\bottomrule
\end{tabular}}%
\begin{minipage}[c]{0.71\textwidth}
\centering
\includegraphics[height=\dimexpr\ht\tablebox+\dp\tablebox\relax]{figs/imagenet/cfg_sweep_sit_ot_vs_ind_xl_2_256_paper_cfg1234_2rows.png}
\end{minipage}\hfill
\begin{minipage}[c]{0.27\textwidth}
\centering
\usebox{\tablebox}
\end{minipage}
\end{table*}

==> table2.tex <==
% \newsavebox\ablationtable

% % preamble (once): \newsavebox\ablationtable
% % needs: \usepackage{multirow}

% \begin{table*}[t]
% \centering
% \caption{\small \textbf{Left:} FID\,$\downarrow$ on ImageNet for independent vs.\ global transport coupling
%          across sampling steps and CFG guidance scales $w$.
%          \textbf{Right:} Qualitative comparison of global transport vs.\ independent coupling
%          for SiT-XL/2 across guidance scales $w$.}
% \label{tab:sit_ablations}
% \vspace{-0.4em}
% % =========================================================
% % Measure the ablation table into a box (resized)
% % =========================================================
% \sbox\ablationtable{%
% \resizebox{0.63\textwidth}{!}{%
% \begin{tabular}{ll *{9}{c}}
% \toprule
%  & & \multicolumn{3}{c}{16 steps} & \multicolumn{3}{c}{32 steps} & \multicolumn{3}{c}{64 steps} \\
% \cmidrule(lr){3-5}\cmidrule(lr){6-8}\cmidrule(lr){9-11}
% Model & Coupling & \multicolumn{1}{c}{$w{=}1.0$} & 2.0 & 4.0 & 1.0 & 2.0 & 4.0 & 1.0 & 2.0 & 4.0 \\
% \midrule
% \multirow{3}{*}{SiT-B/2}
%  & Independent          & 33.29 & 5.88 & 15.37 & 28.33 & 5.32 & 15.78 & 26.58 & 5.22 & 15.84 \\
%  & Global Transport     & 38.08 & \textbf{5.15} & 13.24 & 33.27 & \textbf{4.35} & 13.49 & 31.43 & \textbf{4.14} & 13.54 \\
%  & Class-conditional OT & 33.18 & 5.79 & 15.15 & 28.43 & 5.20 & 15.59 & 26.72 & 5.08 & 15.59 \\
% \midrule
% \multirow{2}{*}{SiT-L/2}
%  & Independent          & 19.53 & 5.50 & 17.56 & 15.30 & 5.74 & 17.86 & 13.85 & 5.85 & 17.89 \\
%  & Global Transport     & 23.77 & \textbf{3.94} & 14.76 & 19.35 & \textbf{3.84} & 15.17 & 17.72 & \textbf{3.88} & 15.17 \\
%  & Class-conditional OT & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
% \midrule
% \multirow{2}{*}{SiT-XL/2}
%  & Independent          & 18.57 & 5.55 & 17.53 & 14.26 & 5.89 & 17.80 & 12.58 & 6.10 & 17.87 \\
%  & Global Transport     & 22.44 & \textbf{3.87} & 14.66 & 17.82 & \textbf{3.82} & 15.03 & 16.11 & \textbf{3.87} & 15.09 \\
% \bottomrule
% \end{tabular}}}%
% % =========================================================
% % Table and figure side by side, vertically centered on the shared baseline
% % =========================================================
% \mbox{%
% \usebox\ablationtable\hspace{0.8em}%
% \raisebox{-0.5\height}{\includegraphics[height=\dimexpr\ht\ablationtable+\dp\ablationtable\relax]{figs/imagenet/cfg_sweep_sit_ot_vs_ind_xl_2_256_paper_cfg1234_2rows.png}}%
% }
% \end{table*}

\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{figs/imagenet/cfg_sweep_sit_ot_vs_ind_xl_2_256_seed5_paper_2rows_w1-6.png}
    \caption{Caption}
    \label{fig:placeholder}
\end{figure}
